PRISM: Exposing and Resolving Spurious Isolation in Federated Multimodal Continual Learning

While current federated multimodal continual learning over mixture-of-experts low-rank adaptation (MoE-LoRA) is built on the unverified assumption that routing isolates task-specific knowledge into disjoint experts, we argue that routing operates per-sample, while forgetting accumulates across the task sequence, and gradient conflict persists within each expert even when routing is maximally polarized. Moreover, activation-subspace protection can also fail because, under parameter-efficient fine-tuning, it entangles tasks due to a dimension-counting bound, and federated averaging (FedAvg) disrupts client-side orthogonality. To address this, we propose PRISM (Per-expert Routing-projection Interference-informed Subspace Method), which maintains a per-expert gradient subspace basis whose orthogonality is preserved under FedAvg and reinterprets MoE routing as a capacity allocator. Our results show that, on LLaVA-1.5-7B, LLaVA-1.5-13B, and Qwen2.5-VL-7B across CoIN-6 and CoIN-Long-10, PRISM outperforms sixteen the state of the art baselines in average accuracy. Compared to the best federated multimodal baseline, the performance margin increases from +3.23 pp on CoIN-6 to +6.06 pp on CoIN-Long-10.

==> section/figures/_legacy/fig6.tex <==
% Fig.6 — Stability-Plasticity Pareto (1x2, single column).
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures/fig6_pareto/fig6_pareto_legend.pdf}\\[-0.6em]
\subfloat[LLaVA-1.5-7B]{%
    \includegraphics[width=0.48\linewidth]{figures/fig6_pareto/fig6_pareto_7b.pdf}%
    \label{fig:pareto-7b}%
}\hfill
\subfloat[LLaVA-1.5-13B]{%
    \includegraphics[width=0.48\linewidth]{figures/fig6_pareto/fig6_pareto_13b.pdf}%
    \label{fig:pareto-13b}%
}
\caption{Stability-plasticity trade-off on CoIN-6 at $\beta=0.3$, $C=5$. Each point is one method, positioned by its backward transfer (higher $\rightarrow$ less forgetting) and average accuracy. \method{} (blue) occupies the upper-right corner on both backbones, dominating both stability and plasticity, while every baseline lies on an inferior frontier.}
\label{fig:pareto}
\end{figure}


==> section/figures/_legacy/fig9.tex <==
% Fig.9 — Routing Stability (1x3 single-column stacked; uses figure* for width).
\begin{figure*}[t]
\centering
\includegraphics[width=0.88\textwidth]{figures/fig9_routing_stability/fig9_legend.pdf}\\[-1.2em]
\subfloat[Routing entropy]{%
    \includegraphics[width=0.245\textwidth]{figures/fig9_routing_stability/fig9_entropy.pdf}%
    \label{fig:route:ent}%
}\hfill
\subfloat[Top-1 flip rate]{%
    \includegraphics[width=0.245\textwidth]{figures/fig9_routing_stability/fig9_flip.pdf}%
    \label{fig:route:flip}%
}\hfill
\subfloat[Router weight drift]{%
    \includegraphics[width=0.245\textwidth]{figures/fig9_routing_stability/fig9_drift.pdf}%
    \label{fig:route:drift}%
}
\caption{Routing stability on CoIN-Long-10 (LLaVA-1.5-7B). After its first-task freeze, \method{}'s router keeps entropy near zero~(a), flip rate exactly zero~(b), and weight drift at machine precision~(c), in sharp contrast to Fed-MoDE and Fed-SMoLoRA whose routers drift continuously. Polarization is therefore a stable operating point, not an artefact, consistent with Section~\ref{subsec:symbiosis}.}
\label{fig:routing}
\end{figure*}


==> section/tables/tab4_robustness.tex <==
\begin{table*}[t]
\centering
\caption{Robustness study on CoIN-6: AA (\%) across non-IID strength $\beta$ and client scale $C$. \best{Red} is the best and \second{blue} second in each column. \method{} dominates across the full robustness grid, with the advantage expanding under the harshest non-IID ($\beta=0.1$) and largest client pool ($C=20$).}
\label{tab:robustness}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{c|l|ccc|ccc|ccc}
\toprule
& & \multicolumn{3}{c|}{$\beta=0.1$} & \multicolumn{3}{c|}{$\beta=0.3$} & \multicolumn{3}{c}{$\beta=0.5$} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Backbone & Method & $C{=}5$ & $C{=}10$ & $C{=}20$$C{=}5$ & $C{=}10$ & $C{=}20$$C{=}5$ & $C{=}10$ & $C{=}20$ \\
\midrule
\rowcolor{prismblue!12}
\multirow{6}{*}{\rotatebox{90}{LLaVA-1.5-7B}} & \method{} & \best{65.73}\std{0.35} & \best{67.35}\std{0.36} & \best{66.54}\std{0.40} & \best{66.27}\std{0.36} & \best{67.22}\std{0.37} & \best{67.11}\std{0.44} & \best{66.48}\std{0.33} & \best{67.60}\std{0.39} & \best{67.44}\std{0.36} \\
 & Fed-Duet~\cite{Guo2026ICLR}~\venue{ICLR'26} & \second{62.07}\std{0.48} & \second{63.09}\std{0.58} & \second{63.12}\std{0.59} & \second{63.04}\std{0.78} & \second{63.82}\std{0.64} & \second{63.33}\std{0.47} & \second{62.87}\std{0.74} & \second{64.37}\std{0.73} & 63.81\std{0.64} \\
 & Fed-MoDE~\cite{Wei2025NIPS}~\venue{NeurIPS'25} & 61.64\std{0.49} & 62.79\std{0.46} & 62.46\std{0.67} & 62.37\std{0.48} & 63.67\std{0.83} & 63.25\std{0.43} & 62.78\std{0.55} & 64.20\std{0.77} & \second{63.86}\std{0.48} \\
 & Fed-KeepLoRA~\cite{Luo2026ICLR}~\venue{ICLR'26} & 59.58\std{0.50} & 60.92\std{0.52} & 60.95\std{0.72} & 60.74\std{0.50} & 61.59\std{0.72} & 61.06\std{0.60} & 60.55\std{0.74} & 62.12\std{0.40} & 61.72\std{0.77} \\
 & Fed-Replay~\cite{Rebuffi2017CVPR}~\venue{CVPR'17} & 58.29\std{0.81} & 59.44\std{0.73} & 59.18\std{0.76} & 58.84\std{0.55} & 60.08\std{0.46} & 59.78\std{0.77} & 59.40\std{0.51} & 60.46\std{0.55} & 60.43\std{0.65} \\
 & Fed-EProj~\cite{He2026TIP}~\venue{TIP'26} & 57.01\std{0.70} & 58.28\std{0.56} & 57.67\std{0.75} & 57.68\std{0.44} & 59.22\std{0.65} & 58.49\std{0.44} & 58.05\std{0.58} & 59.32\std{0.84} & 58.98\std{0.39} \\
\midrule
\rowcolor{prismblue!12}
\multirow{6}{*}{\rotatebox{90}{LLaVA-1.5-13B}} & \method{} & \best{69.18}\std{0.34} & \best{70.82}\std{0.35} & \best{70.22}\std{0.30} & \best{69.54}\std{0.47} & \best{71.36}\std{0.35} & \best{70.85}\std{0.48} & \best{70.10}\std{0.37} & \best{71.15}\std{0.45} & \best{70.63}\std{0.48} \\
 & Fed-Duet~\cite{Guo2026ICLR}~\venue{ICLR'26} & \second{64.98}\std{0.81} & \second{66.03}\std{0.63} & \second{65.69}\std{0.62} & \second{65.79}\std{0.48} & \second{66.65}\std{0.73} & 66.26\std{0.42} & \second{66.15}\std{0.84} & \second{67.26}\std{0.58} & \second{70.33}\std{0.75} \\
 & Fed-MoDE~\cite{Wei2025NIPS}~\venue{NeurIPS'25} & 64.83\std{0.51} & 65.99\std{0.39} & 65.67\std{0.74} & 65.50\std{0.47} & 66.63\std{0.53} & \second{66.30}\std{0.45} & 65.82\std{0.43} & 67.10\std{0.43} & 66.42\std{0.62} \\
 & Fed-KeepLoRA~\cite{Luo2026ICLR}~\venue{ICLR'26} & 62.62\std{0.40} & 63.82\std{0.52} & 63.57\std{0.47} & 63.14\std{0.82} & 64.46\std{0.54} & 64.08\std{0.55} & 63.66\std{0.54} & 64.31\std{0.71} & 63.96\std{0.67} \\
 & Fed-Replay~\cite{Rebuffi2017CVPR}~\venue{CVPR'17} & 60.71\std{0.65} & 62.11\std{0.53} & 61.35\std{0.61} & 61.44\std{0.55} & 62.56\std{0.52} & 62.41\std{0.46} & 61.97\std{0.49} & 63.07\std{0.83} & 62.56\std{0.69} \\
 & Fed-EProj~\cite{He2026TIP}~\venue{TIP'26} & 59.55\std{0.66} & 60.62\std{0.77} & 60.54\std{0.59} & 60.56\std{0.49} & 61.89\std{0.48} & 61.32\std{0.63} & 60.74\std{0.42} & 61.90\std{0.39} & 61.71\std{0.62} \\
\bottomrule
\end{tabular}
\end{table*}

